Near-Perfect Recovery in the One-Dimensional Latent Space Model

Suppose a graph $G$ is stochastically created by uniformly sampling vertices along a line segment and connecting each pair of vertices with a probability that is a known decreasing function of their distance. We ask if it is possible to reconstruct the actual positions of the vertices in $G$ by only observing the generated unlabeled graph. We study this question for two natural edge probability functions -- one where the probability of an edge decays exponentially with the distance and another where this probability decays only linearly. We initiate our study with the weaker goal of recovering only the order in which vertices appear on the line segment. For a segment of length $n$ and a precision parameter $\delta$, we show that for both exponential and linear decay edge probability functions, there is an efficient algorithm that correctly recovers (up to reflection symmetry) the order of all vertices that are at least $\delta$ apart, using only $\tilde{O}(\frac{n}{\delta ^ 2})$ samples (vertices). Building on this result, we then show that $O(\frac{n^2 \log n}{\delta ^2})$ vertices (samples) are sufficient to additionally recover the location of each vertex on the line to within a precision of $\delta$. We complement this result with an $\Omega (\frac{n^{1.5}}{\delta})$ lower bound on samples needed for reconstructing positions (even by a computationally unbounded algorithm), showing that the task of recovering positions is information-theoretically harder than recovering the order. We give experimental results showing that our algorithm recovers the positions of almost all points with high accuracy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> appexp.tex <==
\section{Omitted Details from Section~\ref{sec:exp}}

\begin{lemma*} [Restatement of Lemma~\ref{lem:exdeg}]
    For any vertex $v_i$ which located at position $x_i$ on the segment, if we uniformly sample a vertex $v$ on the segment, then the edge $(v_i,v)$ will be present with probability $\frac{c}{n}(2-e^{-x_i}-e^{x_i-n})$. 
\end{lemma*}
\begin{proof}
    The probability is the expectation of $e^{-|x_i-x|}$ where $x$ is the location of $v$ which is uniformly sampled on the segment. So the probability is 
    \begin{align*} 
        & \int_0^n \frac{c}{n} e^{-|x_i-x|} dx \\
        = & \frac{c}{n}\int_0^{x_i} e^{x-x_i} dx + \frac{c}{n}\int_{x_i}^n e^{x_i-x} dx \\
        = & \frac{c(2 - e^{-x_i} - e^{x_i-n})}{n}
    \end{align*}
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:excom}]
    For any two vertices $v_i$ and $v_j$ which are located at $x_i$ and $x_j$ on the segment with $x_i<x_j$, if we uniformly sample a vertex $v$ on the segment, then $v$ is a common neighbor of $v_i$ and $v_j$ with probability $\frac{c^2}{n}((x_j-x_i+1)e^{x_i-x_j} - \frac{1}{2}(e^{x_i+x_j-2n}+e^{-x_i-x_j}))$.
\end{lemma*}
\begin{proof}
    Let $p(x)$ be the probability that $v$ is a common neighbor of $v_i$ and $v_j$ where $x$ is the location of $v$, then
    $$
    p(x)=
    \begin{cases}
        c^2 \cdot e^{2x-x_i-x_j}, & \mbox{if } x\le x_i \\
        c^2 \cdot e^{x_i-x_j}, & \mbox{if } x_i<x<x_j \\
        c^2 \cdot e^{x_i+x_j-2x}, & \mbox{if } x\ge x_j
    \end{cases}
    $$
    So the overall probability is
    \begin{align*}
        & \int_0^n \frac{1}{n} p(x) dx \\
        = & \frac{c^2}{n}\int_0^{x_i} e^{2x-x_i-x_j}dx + \frac{c^2(x_j-x_i)}{n} e^{x_i-x_j} + \frac{c^2}{n}\int_{x_j}^n e^{x_i+x_j-2x}dx \\
        = & \frac{c^2(x_j-x_i+1)}{n} e^{x_i-x_j}  - \frac{c^2(e^{-x_i-x_j}+e^{x_i+x_j-2n})}{2n}
    \end{align*}
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:exfar}]
    If $m>\frac{2500n \log n}{c^2 \delta^2}$, with probability $1-o(1)$, for any two vertices $v_i$ and $v_j$, (a) if they have no common neighbor, then $\card{x_i-x_j} > 2.5$, and (b) if $\card{x_i-x_j}>n/2$, then they have no common neighbor.
\end{lemma*}

\begin{proof}
    If $\card{x_i-x_j} \le 2.5$, then one of $e^{-x_i-x_j}$ and $e^{x_i+x_j-2n}$ is $O(e^{-n})$, without loss of generality, suppose $e^{x_i+x_j-2n}$ is $O(e^{-n})$. Since $-x_i-x_j<-\card{x_i-x_j}$, $e^{-x_i-x_j}<e^{-\card{x_i-x_j}}$. By Lemma~\ref{lem:excom}, the probability that a random sampled vertex be a common neighbor of $v_i$ and $v_j$ is at least $\frac{c^2(\card{x_i-x_j}+0.5)}{n}e^{-\card{x_i-x_j}} > \frac{c^2}{2n}e^{-2.5} > \frac{c^2}{30n}$. Since $m>\frac{2500n \log n}{c^2 \delta^2}$, the probability that $v_i$ and $v_j$ have no common neighbor is $o(n^{-80})$.

    If $\card{x_i-x_j} > n/2$, the probability that a random vertex be a common neighbor of them is at most $e^{-n/2}$. So with probaiblity $1-o(n^{-100})$, they have no common neighbor.
\end{proof}



==> apppos.tex <==
\section{Omitted Details from Section~\ref{sec:lb}}

\begin{lemma*} [Restatement of Lemma~\ref{lem:veryfar}]
    If $\card{x_i-x_j} \ge n^{0.1}$, then $\card{L_{i,j}} < n^{-100}$.
\end{lemma*}

\begin{proof}
    By definition of $Y$, $d'_{i,j}=\frac{2\delta d_{i,j}}{n}$. So
    $$L_{i,j} \le \log (1-e^{-d_{i,j}}) - \log (1-e^{d'_{i,j}-d_{i,j}}) = \log (1-\frac{e^{d'_{i,j}-d_{i,j}}(1-e^{-d'_{i,j}})}{1-e^{-d_{i,j}}}) < \log (1-\frac{e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}})$$ 
    Since $d_{i,j} \ge n^{0.1}$, $e^{-d_{i,j}}$ and $e^{d'_{i,j}-d_{i,j}}$ are both $o(n^{-100})$. 
    So $L_{i,j} = \log (1- o(n^{-100})) = o(n^{-100})$ by Proposition~\ref{cla:1-y}.
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:lbXij}]
    For any pair of vertices $v_i,v_j$, $e^{-d_{i,j}}(d'^2_{i,j}/2+(1-e^{-d_{i,j}})a/2) < \expect{L_{i,j}} < e^{-d_{i,j}}(d'^2_{i,j}+\frac{2d'^2_{i,j}}{d_{i,j}})$ where $a=\frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}}$.
\end{lemma*}

\begin{proof}
    By definition of $L_{i,j}$, with probability $e^{-d_{i,j}}$, $L_{i,j}=-d'_{i,j}$ and with probability $1-e^{-d_{i,j}}$, $L_{i,j}=\log (1-e^{-d_{i,j}}) - \log (1-e^{-d_{i,j}+d'_{i,j}}) = - \log (\frac{1-e^{-d_{i,j}+d'_{i,j}}}{1-e^{-d_{i,j}}})$. So 
    \begin{align*}
    \expect{L_{i,j}} &=-d'_{i,j}e^{-d_{i,j}}-(1-e^{-d_{i,j}})\log (\frac{1-e^{-d_{i,j}+d'_{i,j}}}{1-e^{-d_{i,j}}}) \\
                     &= -d'_{i,j}e^{-d_{i,j}}-(1-e^{-d_{i,j}})\log (1- \frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}})
    \end{align*}
    by Proposition~\ref{cla:log}, $a=\frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}} < \frac{d'_{i,j}}{d_{i,j}} < 0.5$. 
    Together with Proposition~\ref{cla:1-y},
    $$
    \expect{L_{i,j}}<-d'_{i,j}e^{-d_{i,j}} + e^{-d_{i,j}}(e^{d'_{i,j}}-1)(1+a) < e^{-d_{i,j}}(e^{d'_{i,j}}-d'_{i,j}-1+\frac{d'_{i,j}(e^{d'_{i,j}}-1)}{d_{i,j}}) 
    $$
    Since $d'_{i,j}<1/2$, $e^{d'_{i,j}}<1+d'_{i,j}+d'^2_{i,j}$ and $e^{d'_{i,j}}<1+2d'_{i,j}$. So $\expect{L_{i,j}} < e^{-d_{i,j}}(d'^2_{i,j}+2d'^2_{i,j}/d_{i,j})$.

    Again by Proposition~\ref{cla:1-y},
    \begin{align*}
    \expect{L_{i,j}} &> -d'_{i,j}e^{-d_{i,j}} + e^{-d_{i,j}}(e^{d'_{i,j}}-1)(1+a/2) \\ 
                     &> e^{-d_{i,j}}(e^{d'_{i,j}}-d'_{i,j}-1+(e^{d'_{i,j}}-1)a/2) \\ 
                     &> e^{-d_{i,j}}(d'^2_{i,j}/2 + (e^{d'_{i,j}}-1)a/2)
    \end{align*}
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:ubex}]
    If $m<\frac{(10^{-5})n^{3/2}}{\delta}$ and $X$ is obtained by sampling each point uniformly, then $\expect{\sum_{i,j} L_{i,j}} < 10^{-8}$ with probability $1-o(1)$.
\end{lemma*}

\begin{proof}
    Let the $S_1,S_2,\dots,S_n$ be the set of vertices where $S_k$ contains all the vertices inside the interval $[i,i+1]$ in $X$. Let $i$, $j$ be two vertices inside $S_k$ and $S_{\ell}$ where $k\le \ell$, then $\expect{L_{i,j}} \le 6(\ell-k+1)^2e^{-(\ell-k-1)}\cdot \frac{\delta^2}{n^2}$ by Lemma~\ref{lem:lbXij} and the fact that the distance between $i$ and $j$ is at least $\ell-k-1$ and at most $\ell-k+1$, $\card{y_i-y_j} = (1-\frac{2\delta}{n}) \card{x_i-x_j}$. So
    \begin{align*}
        \expect{\sum_{i,j} L_{i,j}} & = \sum_{k,\ell} \sum_{i \in S_k, j\in S_{\ell}} \expect{L_{i,j}} \\
                                    & \le \frac{\delta^2}{n^2}\sum_{k,\ell} |S_k|\cdot |S_{\ell}| 6(\ell-k+1)^2e^{-(\ell-k-1)} \\
                                    & = \frac{\delta^2}{n^2}\sum_{k=0}^{n-1} \sum_{\ell=1}^{n-k} |S_{\ell}| \cdot |S_{\ell+k}| 6(k+1)^2 e^{-(k-1)}
    \end{align*}
    By Rearrangement inequality \cite{zygmund1953hg}, for any $k$, $\sum_{\ell=1}^{n-k} |S_{\ell}| \cdot |S_{\ell+k}| \le \sum_{\ell=1}^n |S_{\ell}|^2$. So
    \begin{align*}
        \expect{\sum_{i,j} L_{i,j}} & \le \frac{\delta^2}{n^2}(\sum_{k=1}^n |S_k|^2) \cdot (\sum_{k=0}^{n-1} 6(k+1)^2 e^{-(k-1)}) \\
                                    & \le \frac{\delta^2}{n^2}(6e + \sum_{k=0}^\infty (6k^2+24k+24) e^{-k)})(\sum_{k=1}^n |S_k|^2) \\
                                    & \le \frac{\delta^2}{n^2}(6e + \frac{6e(1+e)}{(e-1)^3} + \frac{24e}{(e-1)^2} + \frac{24e}{e-1}) \cdot (\sum_{k=1}^n |s_k|^2) \\                   
                                    & \le \frac{100\delta^2}{n^2}\sum_{k=1}^n |S_k|^2
    \end{align*}
    By the choice of $m$, each $|S_k|<2m/n < \frac{10^{-5}n^{1/2}}{\delta} $ with probability $1-o(1)$ by Chernoff bound, so $\sum_{k=1}^n |S_k|^2 \le \frac{10 ^ {-10} n^2}{\delta^2}$, which means $\expect{\sum_{i,j} L_{i,j}} < 10^{-8}$.
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:anti}]
    $\prob{\card{\bar{L}-\expect{\bar{L}}}>10^{-3}\sqrt{\expect{\bar{L}}}} \ge 0.5$.
\end{lemma*}

\begin{proof}
    For any $i$ and $j$, let $t_{i,j} = (d'_{i,j}-\log(\frac{1-e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}}))/2$. We prove that $t_{i,j}^2(1-Q_{L_{i,j}}(t_{i,j})) \ge \frac{1}{20}\expect{L_{i,j}}$ where $Q_{L_{i,j}}$ is the L{\`e}vy concentration function of $L_{i,j}$ (see Definition~\ref{def:levy}). 

    Sincee $L_{i,j}$ is either $-d'_{i,j}$ or $-\log(\frac{1-e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}})$, $Q_{L_{i,j}}(t_{i,j})$ is the maximum between $e^{-d_{i,j}}$ and $1-e^{-d_{i,j}}$. Also, $2t_{i,j}$ is larger than both $d'_{i,j}$ and $\log(\frac{1-e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}})$. 

    If $e^{-d_{i,j}} \le 1/2$, $d_{i,j} \ge \log 2$, $t_{i,j}^2(1-Q_{L_{i,j}}(t_{i,j})) \ge \frac{1}{4}(d'^2_{i,j} e^{-d_{i,j}})$, which is larger than $\frac{1}{20}(1+2/d_{i,j})d'^2_{i,j}e^{-d_{i,j}} > \frac{1}{16}\expect{L_{i,j}}$ sincee $d_{i,j}>\log 2$ and Lemma~\ref{lem:lbXij}. 

    Otherwise $e^{-d_{i,j}} > 1/2$, $t_{i,j}^2(1-Q_{L_{i,j}}(t_{i,j})) \ge \frac{1}{4}((1-e^{-d_{i,j}}) \log^2(\frac{1-e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}})$. Let $a = \frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}}$, By Lemma~\ref{lem:lbXij}, $\expect{L_{i,j}}=-d'_{i,j}e^{-d_{i,j}}-(1-e^{-d_{i,j}})\log (1-a) >0$, so $-(1-e^{-d_{i,j}})\log (1-a)>d'_{i,j}e^{-d_{i,j}}$, which means 
    $$(1-e^{-d_{i,j}}) \log^2(\frac{1-e^{d'_{i,j}-d_{i,j}}}{1-e^{-d_{i,j}}}) = (1-e^{-d_{i,j}}) \log^2 (1-a) > -d'_{i,j}e^{-d_{i,j}} \log (1-a)> a d'_{i,j}e^{-d_{i,j}}$$
    Since $e^{-d_{i,j}} > 1/2 > 1-e^{-d_{i,j}}$, $a = \frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}} > e^{d'_{i,j}}-1 > d'_{i,j}$, also $a = \frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}} > \frac{e^{d'_{i,j}}-1}{2(1-e^{-d_{i,j}})} > \frac{d'_{i,j}}{2d_{i,j}}$. So $5a > d'_{i,j} + 2d'_{i,j}/d_{i,j}$, which means 
    $$t_{i,j}^2(1-Q_{L_{i,j}}(t_{i,j})) \ge \frac{1}{4}d'_{i,j}e^{-d_{i,j}} a > \frac{1}{20}d'^2_{i,j} (1+2/d_{i,j})e^{-d_{i,j}} > \frac{1}{20} \expect{L_{i,j}}$$ 
    by Lemma~\ref{lem:lbXij}. 

    By Proposition~\ref{prop:KR}, 
    $$
    Q_{\bar{L}}(10^{-3}\sqrt{\expect{\bar{L}}}) \le \frac{10^{-1} \sqrt{\expect{\bar{L}}}}{\sqrt{\sum_{i \sim j}t_{i,j}^2Q_{L_{i,j}}(t_{i,j})}} \le \frac{0.1\sqrt{\expect{\bar{L}}}}{\sqrt{0.05\sum_{i \sim j}\expect{L_{i,j}}}} \le 0.5
    $$
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:lbsubexp}]
    For any pair of $i$ and $j$, if $d_{i,j} < n^{0.1}$, then $L_{i,j}$ is a sub-exponential variable with parameters $(\sigma_{i,j},b)$ where $\sigma_{i,j}^2=48\expect{L_{i,j}}$ and $b=n^{-0.8}$.
\end{lemma*}

\begin{proof}
    By Proposition~\ref{cla:subexp}, it is sufficient to prove for any $\card{\lambda}<n^{0.8}$,
    $$
    \expp{L_{i,j},L'_{i,j}}{e^{\frac{\lambda^2(L_{i,j}-L'_{i,j})^2}{2}}} < e^{\frac{\lambda^2\sigma_{i,j}^2}{2}}
    $$
    Where $L'_{i,j}$ is a random variable independent and identical to $L_{i,j}$.

    Again, by convenience, denote $a = \frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}}$. We first bound $\card{L_{i,j}}$, $L_{i,j}$ is either $-d'_{i,j}$ or $-\log(1-a)$ where $d'_{i,j}$ = $\frac{2d_{i,j}\delta}{n} = o(n^{-0.8})$. Also by Proposition~\ref{cla:1-y} and Proposition~\ref{cla:log}, $-\log(1-a) < a + a^2 < \frac{d'_{i,j}}{d_{i,j}} + \frac{d'^2_{i,j}}{d_{i,j}^2} < \frac{2\delta}{n} = o(n^{-0.8})$. So $L_{i,j}-L'_{i,j} = o(n^0.8)$. So $\lambda^2(L_{i,j}-L'_{i,j})^2 = o(1)$ for any $\card{\lambda}<n^{0.8}$. So
    $$
    \expp{L_{i,j},L'_{i,j}}{e^{\frac{\lambda^2(L_{i,j}-L'_{i,j})^2}{2}}} < 1 + \expp{L_{i,j},L'_{i,j}}{\lambda^2(L_{i,j}-L'_{i,j})^2}
    $$
    On the other hand,
    $$
    e^{\frac{\lambda^2\sigma_{i,j}^2}{2}} > 1 + \frac{\lambda^2\sigma_{i,j}^2}{2}
    $$
    To prove the lemma, it's sufficient to prove $\sigma_{i,j}^2 > 2\expp{L_{i,j},L'_{i,j}}{(L_{i,j}-L'_{i,j})^2}$. By definition of $L_{i,j}$, 
    \begin{align*}
    \expp{L_{i,j},L'_{i,j}}{(L_{i,j},L'_{i,j})^2} 
        &= 2e^{-d_{i,j}}(1-e^{-d_{i,j}})(d'_{i,j}-\log(1-a))^2 \\
        &< 4e^{-d_{i,j}}d'^2_{i,j} + 4(1-e^{-d_{i,j}})\log^2(1-a)
    \end{align*}
    By Proposition~\ref{cla:1-y} and Proposition~\ref{cla:log}, $a<1/2$ and $\log^2(1-a) < (a+a^2)^2 < 3a^2$. So
    $$
    4e^{-d_{i,j}}d'^2_{i,j} + 4(1-e^{-d_{i,j}}) \log^2(1-a) <4e^{-d_{i,j}}(d'^2_{i,j}+3(e^{d'_{i,j}}-1)a)<24\expect{L_{i,j}}
    $$
    by Lemma~\ref{lem:lbXij}. The proof finish with $\sigma_{i,j}^2 = 48\expect{L_{i,j}}$.
\end{proof}

\begin{lemma*} [Restatment of Lemma~\ref{lem:losum}]
    If $1000n< m < \frac{(10^{-5})n^{3/2}}{\delta}$, then $\expect{\bar{L}} = \omega(n^{-1.6})$.
\end{lemma*}

\begin{proof}
    By Chernoff bound, if $m>1000n$, with probability $1-o(1)$, there is a vertex in any segments with length $\frac{\log n}{20}$. Without loss of generality, suppose $x_1<x_2<\dots<x_m$, then $x_{i+1}-x_i < \frac{\log n}{10}$ for any $i$ and $x_m-x_1>n-\log n > 0.9n$. So by Lemma~\ref{lem:lbXij},
    $$
    \expect{\bar{L}} > \sum_{i=1}^{m-1} \expect{L_{i,i+1}} > e^{-\frac{\log n}{20}} \sum_{i=1}^{m-1} (\frac{2\delta(x_{i+1}-x_i)}{n})^2 = \omega(n^{-2.1}) \sum_{i=1}^{m-1} (x_{i+1}-x_i)^2
    $$
    By Cauchy-Schwarz inequality, 
    $$
    \sum_{i=1}^{m-1} (x_{i+1}-x_i)^2 > \frac{1}{m} (\sum_{i=1}^{m-1} (x_{i+1}-x_i))^2 > \frac{1}{m} (0.9n)^2 = \Omega(n^{0.5})
    $$
    So $\expect{\bar{L}} = \omega(n^{-1.6})$.
\end{proof}

\begin{lemma*} [Restatment of Lemma~\ref{lem:lbcon}]
    If $1000n < m < \frac{(10^{-5})n^{3/2}}{\delta}$, then for any integer $k>0$, $\prob{\card{\bar{L}-\expect{\bar{L}}} > 10k \sqrt{\expect{L}}} < 4 e^{-k}$.
\end{lemma*}

\begin{proof}
    By Proposition~\ref{prop:Hof} and Lemma~\ref{lem:lbsubexp}, 
    $$
    \prob{\card{\bar{L}-\expect{\bar{L}}} > 10k \sqrt{\expect{\bar{L}}}} < 2 e^{-\frac{100k^2\expect{\bar{L}}}{2\sigma_{\star}^2}} + 2 e^{-\frac{10k\sqrt{\expect{\bar{L}}}}{2b}}
    $$
    where $\sigma_{\star}^2 = \sum_{i~j} \sigma_{i,j}^2 = 48 \expect{\bar{L}}$ and $b=n^{-0.8} < \sqrt{\expect{\bar{L}}}$ by Lemma~\ref{lem:losum}.
    So
    $$
    2 e^{-\frac{100k^2\expect{\bar{L}}}{2\sigma_{\star}^2}} + 2 e^{-\frac{10k\sqrt{\expect{\bar{L}}}}{2b}} < e^{-\frac{100k^2}{96}} + 2e^{-\frac{10k}{2}} < 4 e^{-k}
    $$
\end{proof}

\section{Omitted Details from Section~\ref{sec:ub}}

\begin{lemma*} [Restatement of Lemma~\ref{lem:ubfar}]
If $m = \tilde{O}(n^2)$, with probability $1-o(1)$, for any pair of $(i,j)$, $\card{x_i-x_j}>\frac{1}{n^4}$.
\end{lemma*}

\begin{proof}
For any pair of $(i,j)$, the probability that $\card{x_i-x_j} \le \frac{1}{n^4}$ is at most $\frac{\frac{2}{n^4}}{n} = O(\frac{1}{n^5})$. Since there are at most $m^2 = o(n^5)$ pair of $(i,j)$, so with probability $1-o(1)$ there is no such $(i,j)$.
\end{proof}

\begin{lemma*} [Restatement of Lemma~\ref{lem:ubsubexp}]
For those pair of $(i,j)$ contribute to $\bar{L}$, $\bar{L}_{i,j}$ is a sub-exponential random variable with parameter $(\sigma_{i,j},b)$ where $\sigma_{i,j}^2 = 10 \log n \cdot \expect{\bar{L}_{i,j}}$ and $b = 10 \log n$.
\end{lemma*}

\begin{proof}
By Proposition~\ref{cla:subexp}, it is sufficient to prove that for any $\lambda<\frac{1}{b}$, 
$$
\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{e^{\frac{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2}{2}}} < e^{\frac{\lambda^2\sigma_{i,j}^2}{2}}
$$
where $\bar{L}'_{i,j}$ is a random varibale independent and identical to $\bar{L}_{i,j}$.
We prove the lemma respectively in the case of $\card{y_i-y_j} \le \card{x_i-x_j}$ and $\card{y-i-y_j} < \card{x_i-x_j}$.

\textbf{Case 1:} $\card{y_i-y_j} \le \card{x_i-x_j}$. Denote $a=\frac{e^{-d_{i,j}}(e^{d'_{i,j}}-1)}{1-e^{-d_{i,j}}}$. $\bar{L}_{i,j} = -d'_{i,j}$ with probability $e^{-d_{i,j}}$ and $a + \frac{1}{2} a^2$ with probability $(1-e^{-d_{i,j}})$. So 
\begin{align*}
\expect{\bar{L}_{i,j}} &= -d'_{i,j}e^{-d_{i,j}} + (1-e^{-d_{i,j}})(a+\frac{1}{2} a^2) \\
                       &= e^{-d_{i,j}}(e^{d'_{i,j}}-d_{i,j}-1) + \frac{1}{2} (1-e^{-d_{i,j}})a^2 \\
                       &\ge \frac{1}{2}(e^{-d_{i,j}} d'^2_{i,j} + (1-e^{-d_{i,j}}) a^2)
\end{align*}
So $e^{\frac{\lambda^2\sigma^2}{2}} > 1 + 5\lambda^2 e^{-d_{i,j}} (d'^2_{i,j} +a^2) \log n$.

On the other hand, $(\bar{L}_{i,j}-\bar{L}'_{i,j})^2 = (d'_{i,j}+a)^2 \le 2d'^2_{i,j}+2a^2$ with probability $2e^{-d_{i,j}}(1-e^{-d_{i,j}}$ and $0$ otherwise. By the condition that $\bar{L}_{i,j}$ contributes to $\bar{L}$, $d'_{i,j} \le d_{i,j} \le 5 \log n$; by Proposition~\ref{cla:log}, $a \le 1$. So $\lambda^2(2d'^2_{i,j}+2a^2) < \frac{50 \log^2 n + 2}{100\log ^2 n} < 1$ for any $\lambda<\frac{1}{b}$. Which means
\begin{align*}
\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{e^{\frac{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2}{2}}} 
    &\le 1 + \expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} \\
    &\le 1 + 2e^{-d_{i,j}}(1-e^{-d_{i,j}})(2d'^2_{i,j}+2a^2)\lambda^2
\end{align*}
which means
$$
\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{e^{\frac{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2}{2}}} < e^{\frac{\lambda^2\sigma_{i,j}^2}{2}}
$$

\textbf{Case 2:} $\card{y_i-y_j} > \card{x_i-x_j}$. Denote $a = \log (\frac{1-e^{-(d_{i,j}+d'_{i,j})}}{1-e^{-d_{i,j}}})$. $\bar{L}_{i,j} = \min \{d'_{i,j},2\}$ with probability $e^{-d_{i,j}}$ and $-a$ with probability $(1-e^{-d_{i,j}})$. Since $d_{i,j} \ge \frac{1}{n^4}$, $\log (1-e^{-d_{i,j}}) \ge \log (1-e^{-n^{-4}}) \ge \log (\frac{1}{2n^4}) \ge -5\log n$, which means $a<5\log n$. So $\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2 \le (2a^2+2)\lambda^2 < 1$ for any $\lambda<\frac{1}{10\log n} = \frac{1}{b}$. So
$$
\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{e^{\frac{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2}{2}}} \le 1 + \expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{\lambda^2(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} 
$$
On the other hand, $e^{\frac{\lambda^2\sigma^2}{2}} > 1 + 5\lambda^2\expect{\bar{L}_{i,j}} \log n$, so we just need to prove 
$$\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} \le 5\expect{\bar{L}_{i,j}} \log n$$

\textbf{Case 2.1:} If $d'_{i,j} \ge 2$, 
\begin{align*}
\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} 
    &= 2e^{-d_{i,j}}(1-e^{-d_{i,j}})(8+2a^2) < 16e^{-d_{i,j}} + 4(1-e^{-d_{i,j}})a \log n \\
    &< 16e^{-d_{i,j}} + 4e^{-d_{i,j}}(1-e^{-d'_{i,j}}) \log n < 5e^{-d_{i,j}} \log n
\end{align*}
On the other hand, $\expect{\bar{L}_{i,j}} = 2 e^{-d_{i,j}} - (1-e^{-d_{i,j}})a > e^{-d_{i,j}} (2 - (1-e^{-d'_{i,j}})) > e^{-d_{i,j}}$, so $5\expect{\bar{L}_{i,j}} \log n > 5e^{-d_{i,j}} \log n$. 

\textbf{Case 2.2:} If $d'_{i,j} \le d_{i,j}$ and $d'_{i,j} < 2$,
$\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} < 2e^{-d_{i,j}}(1-e^{-d_{i,j}})(2d'^2_{i,j}+2a^2) $. Let $z = \frac{e^{-d_{i,j}}(1-e^{-d'_{i,j}})}{1-e^{-d_{i,j}}}$, by Proposition~\ref{cla:log2}, $z<\frac{d'_{i,j}}{d_{i,j}} \le 1$, so $a = \log (1+z) < z - \frac{z^2}{2} + \frac{z^3}{3} < z-\frac{z^2}{6}$, which means $\expect{\bar{L}_{i,j}} > e^{-d_{i,j}}d'_{i,j} - (1-e^{-d_{i,j}})(z-\frac{z^2}{6}) = e^{-d_{i,j}}(d'_{i,j}+e^{-d'_{i,j}}-1)+\frac{1}{6}z^2(1-e^{-d_{i,j}})$ where $e^{-d'_{i,j}}+d'_{i,j}-1 > \frac{d'^2_{i,j}}{2} - \frac{d'^3_{i,j}}{6} > \frac{d'^2_{i,j}}{6}$ since $d'_{i,j} < 2$. So $\expect{\bar{L}_{i,j}} > \frac{1}{6}e^{-d_{i,j}}d'^2_{i,j} + \frac{1}{6}z^2(1-e^{-d_{i,j}})$. On the other hand, $2e^{-d_{i,j}}(1-e^{-d_{i,j}})(2d'^2_{i,j}+2a^2)<4e^{-d_{i,j}}d'^2_{i,j}+4(1-e^{-d_{i,j}})z^2$. So $\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} < \expect{\bar{L}_{i,j}} \cdot \log n$.

\textbf{Case 2.3:} If $d_{i,j} < d'_{i,j} < 2$, let $\eps=e^{-d_{i,j}} \frac{d'_{i,j}}{d_{i,j}}$ and $z = \frac{e^{-d_{i,j}}(1-e^{-d'_{i,j}})}{1-e^{-d_{i,j}}}$. Since $a=\log (1+z) < z$, $\expect{\bar{L}_{i,j}} > e^{-d_{i,j}}(d'_{i,j}- 1 + e^{-d'_{i,j}}) > \frac{1}{6} e^{-d_{i,j}} d'^2_{i,j}$ since $d'_{i,j}<2$. On the other hand, since $d'_{i,j}>d_{i,j}$, $\frac{1-e^{-d'_{i,j}}}{1-e^{-d_{i,j}}} < \frac{d'_{i,j}}{d_{i,j}}$ by Proposition~\ref{cla:log3}, so $a< \log (1+e^{-d_{i,j}}\frac{d'_{i,j}}{d_{i,j}}) = \log (1+\eps)$, and $\expect{\bar{L}_{i,j}} > d_{i,j} \eps - (1-e^{-d_{i,j}}) \log (1+\eps) > d_{i,j} (\eps - \log (1+\eps)) > \frac{d_{i,j}}{2}\log (1+\eps)^2$ (the last inequality is due to $e^a-a-1>\frac{a^2}{2}$ for any $a>0$). So
$$
\expect{\bar{L}_{i,j}} > \frac{1}{2}(\frac{1}{6}e^{-d_{i,j}} d'^2_{i,j} + \frac{d_{i,j}}{2} \log(1+\eps)^2) > \frac{1}{24}(e^{-d_{i,j}}(1-e^{-d_{i,j}}) ( d'^2_{i,j} + 3 a^2) )
$$
So
$$\expp{\bar{L}_{i,j},\bar{L}'_{i,j}}{(\bar{L}_{i,j}-\bar{L}'_{i,j})^2} \le 4e^{-d_{i,j}}(1-e^{-d_{i,j}})(d'^2_{i,j} + a^2) \le 5\expect{\bar{L}_{i,j}} \log n$$

\end{proof}

The following lemma shows that $d'_{i,j}$ satisfies the triangle inequality.

\begin{lemma} \label{lem:ubtri}
For any $i$, $j$ and $k$, $d'_{i,j} \le d'_{i,k}+d'_{k,j}$.
\end{lemma}

\begin{proof}
Since $X$ and $Y$ has the same vertex order, $d'_{i,k}+d'_{k,j} = \card{x_i-x_k-y_i+x_k} + \card{x_j-x_k-y_j+y_k} \ge \card{x_i-x_j-y_i+y_j} = d'_{i,j}$.
\end{proof}


\begin{lemma*} [Restatement of Lemma~\ref{lem:ubexp}]
If $\frac{100n^{1.5} \log n}{\delta} < m = \Omega({n^2})$. If $X$ is sampled uniformly, then with probability $1-o(1)$, for any $Y$ such that there is a pair of $i$ and $j$ satisfies that $d'_{i,j}> \frac{\delta}{2}$,  $\expect{\bar{L}}>5 \log^2 n$.
\end{lemma*}

\begin{proof}
By Lemma~\ref{lem:lbLij}, $\expect{\bar{L}_{i,j}} \ge 0$. It is sufficient to prove that sum of some $\expect{\bar{L}_{i,j}}$ contributed to $\bar{L}$ is larger than $5 \log n$. We first prove that if there is a pair of $i'$ and $j'$ satisfies $d_{i',j'} \le 1$ and $d'_{i',j'}>\frac{\delta}{8}$, then $\expect{\bar{L}}>5\log^2 n$. By Chernoff bound, with probability $1-o(1)$ there are at least $\frac{90\sqrt{n} \log n}{\delta}$ vertices in each segment of length $1$. So there are at least $\frac{90\sqrt{n}\log n}{\delta}$ vertices which is at most $1$ away from both $v_{i'}$ and $v_{j'}$. Suppose $v_k$ is such a vertex, then either $d'_{i',k}$ or $d'_{k,j'}$ is at least $\frac{\delta}{16}$ by Lemma~\ref{lem:ubtri}, which means either $\expect{\bar{L}_{i',k}}$ or $\expect{\bar{L}_{k,j'}}$ is at least $\frac{\delta^2}{256e}$ by lemma~\ref{lem:lbLij}. So $\bar{L}>\frac{90\sqrt{n}\log n}{\delta} \cdot \frac{\delta^2}{256e} > 5 \log^2 n$. 

For any integer $K$, let $S_{K}$ be the set of vertex in segment $[K-1,K]$. Let $v_i \in S_I$ and $v_j \in S_J$. Without loss of generality, suppose $I \le J$. Then for any vertex $v_k$ in $S_I$ (resp. $S_j$), if $d'_{i,k}$ (resp. $d'_{k,j}$) is at least $\frac{\delta}{8}$, which means $\expect{L}>5 \log^2 n$. Otherwise, we have $I<J$ and for any $v_k \in S_I$ and $v_{\ell} \in S_J$, $d'_{k,\ell}> \frac{\delta}{4}$. 

For any $I \le K \le J$, let $v_{k_{K}}$ be an arbitrary vertex in $S_K$. We prove that $\sum_{I\le K < J} \expect{\bar{L}_{k_K,k_{K+1}}} \ge \frac{\delta^2}{1000n}$. For any $K$, since $v_{k_K}$ and $v_{k_{K+1}}$ are in $S_K$ and $S_{K+1}$ respectively, $d_{k_K,k_{K+1}} \le 2$, which means $e^{-d_{k_K,k_{K+1}}} > e^{-2} > \frac{1}{10}$. If there exists a $K$ such that $d'_{k_K,k_{K+1}} > 2$, then $\bar{L}_{k_K,k_{K+1}} > \frac{1}{10} > \frac{\delta^2}{1000n}$ by Lemma~\ref{lem:ubexp}. Otherwise $\sum_{I\le K < J} \expect{\bar{L}_{k_K,k_{K+1}}} \ge \frac{1}{60} \sum_{I \le K < J} d'^2_{k_K,k_{k+1}}$ by Lemma~\ref{lem:ubexp}. Since $d'_{k_I,k_J}>\frac{\delta}{4}$, $\sum_{I \le K <j} d'_{k_K,k_{k+1}} \ge \frac{\delta}{4}$ by Lemma~\ref{lem:ubtri}. By Cauchy-Schwarz inequality, 
$$
\sum_{I \le K <j} d'^2_{k_K,k_{k+1}} \ge \frac{1}{J-I} (\sum_{I \le K <j} d'_{k_K,k_{k+1}})^2 \ge \frac{\delta^2}{16(J-I)} \ge \frac{\delta^2}{16n}
$$
which means $\sum_{I\le K < J} \expect{\bar{L}_{k_K,k_{K+1}}} \ge \frac{\delta^2}{1000n}$.


Let $N=\frac{90\sqrt{n}}{\delta}$ and for any $I \le K \le J$, let $v_{\ell^K_1},v_{\ell^K_2},\dots,v_{\ell^K_N}$ be arbitrary $N$ vertices in $S_k$. Then
\begin{align*}
\expect{\bar{L}} &\ge \sum_{I \le K <J} \sum_{i'=1}^N \sum_{j'=1}^N \expect{\bar{L}_{\ell^K_{i'}, \ell^{K+1}_{j'}}}  = \sum_{I \le K <J} \sum_{i'=1}^N \sum_{j'=0}^{N-1} \expect{\bar{L}_{\ell^K_{i'}, \ell^{K+1}_{(i'+j') \mod N + 1 }}}\\
                 &= \sum_{i'=1}^N \sum_{j'=0}^{N-1} \sum_{I \le K < J} \expect{\bar{L}_{\ell^K_{(i' + Kj') \mod N +1}, \ell^{K+1}_{(i'+(K+1)j') \mod N + 1 }}}\\
                 &\ge \sum_{i'=1}^N \sum_{j'=0}^{N-1} \frac{\delta^2}{1000n} = \frac{N^2 \delta^2}{1000n} > 5 \log^2 n
\end{align*}
\end{proof}



==> prelim.tex <==
\newcommand{\expp}[2]{\mathbb{E}_{#1}\bracket{#2}}

\section{Preliminaries}

\iffalse
\subsection{Problem Statement}


%{\bf Sanjeev: Throughout, it should be $\hat{x}_i$ and not $\hat{x_i}$. It should be ``poly''and not ``Poly''.}


We consider the following problem: On the segment $[0,n]$ $m$ points, say $v_1,v_2,\dots,v_m$, are uniformly sampled. Let $x_i$ be the location of $v_i$, and let $X=(x_1,x_2,\dots,x_m)$ be the location vector. A random graph $G$ is constructed with this vertex set;  edges are sampled independently as follows: for any pair of vertices $v_i$ and $v_j$, an edge exists between them with probability $c \cdot f(\card{x_i-x_j})$, where $c$ is a number in $(0,1]$ and $f$ is some monotone decreasing function such that $f(0)=1$ and $\lim_{x \rightarrow \infty} f(x)=0$. For such a graph $G$ and a position vector $X$, denote by $P_X(G)$ the likelihood of $G$ given $X$, i.e. $P_X(G) = \prod_{(i,j)\in G} c \cdot f(\card{x_i-x_j}) \cdot \prod_{(i,j)\notin G} (1-c \cdot f(\card{x_i-x_j}))$.

Our goal is to design an algorithm that takes as input the graph $G$, and a constant $\delta$, and outputs  a vector $(\hat{x}_1,\hat{x}_2,\dots,\hat{x}_m)$ which is a ``recovery'' of the location of each point. We consider two distinct notions of recovery: (1) recovering the order, by which we mean that for any pair of $i$ and $j$ such that $x_i-x_j > \delta$, $\hat{x}_i > \hat{x}_j$ with high probability; (2) recovering the location, by which we mean that  for any $i$, $\card{x_i-\hat{x}_i}<\delta$ with high probability. 

For the problem of recovering the order, we consider two natural choices of $f$, which are the function $f(x)=e^{-x}$, and the function $f(x) = \frac{1}{x+1}$. For both these cases, we prove that to recover the order, we only need $m = \tilde{O}(\frac{n}{\delta^2})$ points. Notice that $\Omega(n \log n)$ points are necessary, since otherwise $G$ will have isolated vertices  with high probability, and there is no way to recover the relative position of these vertices.

For the problem of recovering the location, we only consider $f(x)=e^{-x}$ in the special case when $c=1$. Modifying the argument for recovering the order, we can show that we can recover locations with  $m=O(n^2\log n/\delta^2)$ points. On the other hand, for any $m = o(n^{1.5}/\delta)$, we give two location vectors $X^1$ and $X^2$ such that $\norm{X^1-X^2}_{\infty} > \delta$ and prove that it is impossible to distinguish these two vectors with large constant probability given the random graph $G$. This suggests that  $\Omega(n^{1.5}/\delta)$ points are necessary to recover locations. However, given $m=\Omega(n^{1.5}\log n/\delta)$ samples, we prove that we can distinguish between any two location vector $X^1$ and $X^2$ such that $\norm{X^1-X^2}_\infty > \delta$.  Note that the $\tilde{O}(n^{1.5})$ upper bound refers to the problem of distinguishing two position vectors. The best upper bound we can prove for recovering position is still $\tilde{O}(n^2)$.
\fi


We first prove a simple statement --- that with enough samples, each segment of length $\delta$ has at least one vertex. {\color{red}Note that in this paper, whenever we say $1 - o(1)$, we mean $1 - 1/poly(n)$.}

\begin{lemma} \label{lem:uniform}
If $m>\frac{8n\log n}{\delta^2}$ and $\delta<1$, with probability $1-o(1)$, for any non-negative integer $i$, the segment $[\frac{i\delta}{2},\frac{(i+1)\delta}{2}]$ on the segment has at least one point.
\end{lemma}
\begin{proof}
Since $\log (\frac{1}{\delta}) < \frac{1}{\delta}-1$, $m>\frac{8n \log n + 8n \log n \log (\frac{1}{\delta})}{\delta} > \frac{8n\log (\frac{n}{\delta})}{\delta}$. For any such segment, the probability that there is no point on it is $(1-\frac{\delta}{2n})^m < e^{-\frac{m \delta}{4 n}} = o(\frac{\delta}{n})$. The assertion follows by using the union bound  over all segments.
%\sampath{But there are $\frac{n}{\delta}$ such segments... so union bound doesn't work.  Do we need a factor $\log (1/\delta)$ more samples?}
\end{proof}
